Evaluating Quantized Large Language Models

Post-training quantization (PTQ) has emerged as a promising technique to reduce the cost of large language models (LLMs). Specifically, PTQ can effectively mitigate memory consumption and reduce computational overhead in LLMs. To meet the requirements of both high efficiency and performance across diverse scenarios, a comprehensive evaluation of quantized LLMs is essential to guide the selection of quantization methods. This paper presents a thorough evaluation of these factors by evaluating the effect of PTQ on Weight, Activation, and KV Cache on 11 model families, including OPT, LLaMA2, Falcon, Bloomz, Mistral, ChatGLM, Vicuna, LongChat, StableLM, Gemma, and Mamba, with parameters ranging from 125M to 180B. The evaluation encompasses five types of tasks: basic NLP, emergent ability, trustworthiness, dialogue, and long-context tasks. Moreover, we also evaluate the state-of-the-art (SOTA) quantization methods to demonstrate their applicability. Based on the extensive experiments, we systematically summarize the effect of quantization, provide recommendations to apply quantization techniques, and point out future directions. The code can be found in https://github.com/thu-nics/qllm-eval.

==> ICML24/Sections/conclusion.tex <==
% \vspace{-10pt}
\section{Conclusion and Potential Broader Impacts}
\label{sec:conclusion}
In this paper, we summarize the status quo of quantized LLMs.
Specifically, we summarize the phenomena of quantization on three tensor types, various LLM families, and different tasks.
Drawing from our evaluation results, we offer suggestions on how to choose and apply quantization techniques and point out the necessity of studying how to quantize MoE models and how to quantize models for long-context and math tasks. By presenting a thorough understanding of current trends, we expect our work to benefit future applications and research of LLM quantization. Our work also provides an early evaluation of the influences of efficiency techniques on trustworthiness, which is worth a more thorough investigation.

%Additionally, we point out directions to mitigate the bad effects of quantization on math, and long-context tasks and MoE models call for future work.

% Given our evaluations of various quantized LLMs on many tasks, we provide the following potential future directions to further explore the effects of quantization:
% (2) It is essential to explore how to reduce the performance loss of quantized models on more challenging tasks, such as mathematical reasoning tasks.
% (3) Further research is needed to delve into improving the performance of quantized models on long-text tasks, especially on KV Cache quantization.
% \todo{(1) Evaluations with more Quantization-Aware Training methods. Can specific abilities be preserved through QAT? }

% \todo{Code Generation task, QAT method Evaluation}

==> ICML24/Sections/efficiency.tex <==
\section{Efficiency Analysis}
\label{sec:efficiency}

In this section, we discuss the efficiency bounds during the inference of LLMs. 
We need to quantize different tensor types to accelerate the operators with different bounds. 
Specifically, we use the Roofline model~\cite{roofline} to analyze the effect of quantizing different tensor types.

% \subsection{Analysis of the Latency Bound}
% \subsection{Analysis of the Memory Consumption}



==> ICML24/Sections/eval_basic.tex <==


\begin{table*}[t]
    \centering
    \caption{The statistical results of Weight, Activation, and KV Cache on OPT, and LLaMA2. Specifically, the statistical results of Activation and KV Cache tensors are calculated using the pile-val dataset. We average each statistical metric across all layers.}
    \vspace{-5pt}
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
    \multirow{2}{*}{Model}   & \multicolumn{3}{c}{Weight} & \multicolumn{3}{c}{Activation} & \multicolumn{3}{c}{KV Cache}  \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    & AbsMax & Std & Kurtosis & AbsMax & Std & Kurtosis & AbsMax & Std & Kurtosis \\
    \midrule
    OPT-1.3B    & 0.27 & 0.02 & 13.16 & 31.20 & 0.72 & \cellcolor{red!20}544.97 & 11.49 & 1.88 & 7.53 \\
    OPT-6.7B    & 0.16 & 0.02 & 8.74 & 44.55 & 0.72 & \cellcolor{red!40}1562.67 & 10.25 & 1.71 & 6.38 \\
    OPT-66B     & 0.11 & 0.01 & 5.19 & 64.36 & 0.71 & \cellcolor{red!80}4945.32  & 13.22 & 2.91 & 7.40 \\
    LLaMA2-7B   & 0.54 & 0.02 & 4.93 & 27.11 & 0.30 & 1167.38 & 11.99 & 0.98 & 14.58 \\
    LLaMA2-70B  & 0.52 & 0.02 & 4.83 & 27.02 & 0.22 & 1279.15 & 11.22 & 1.07 & 10.79 \\
    % Mistral-7B  & 0.08 & 0.03 & 4.01 & 122.33 & 1.74 & 1182.44 & 11.61 & 1.12 & 8.96 \\
    % Mixtral-8x7B  & 0.40 & 0.01 & 4.73 & 63.21 & 1.05 & 176.71 & 16.06 & 1.44 & 11.56 \\
    \bottomrule
    \end{tabular}}
    \label{tab:eval_basic_statistic}
\end{table*}
% 23125.05
% 49239.16

\begin{table*}[t]
    \centering 
    \caption{The statistical results on different linear types in the LLaMA2 family. Q, K, V, and O represent the Query, Key, Value, and Out linear layers in Attention. Gate, Up, and Down represent the three linear layers in FFN.}
    \vspace{-5pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{W or A} & \multicolumn{2}{c}{Q} & \multicolumn{2}{c}{K} & \multicolumn{2}{c}{V} & \multicolumn{2}{c}{O} & \multicolumn{2}{c}{Gate} & \multicolumn{2}{c}{Up} & \multicolumn{2}{c}{Down} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}
    & & Kuro. & Std & Kuro. & Std & Kuro. & Std & Kuro. & Std & Kuro. & Std & Kuro. & Std & Kuro. & Std \\
    \midrule
    \multirow{2}{*}{LLaMA2-7B} & W & 6.95 & 0.02 & 5.37 & 0.02 & 3.33 & 0.02 & \cellcolor{red!40}8.00 & 0.02 & 3.66 & 0.02 & 3.32 & 0.02 & 3.80 & 0.02 \\
    & A & 164.08 & 0.42 & 164.08 & 0.42 & 164.08 & 0.42 & 246.94 & 0.11 & 15.37 & 0.28 & 15.37 & 0.28 & \cellcolor{red!40}1.54e5 & 0.21 \\
    \midrule
    \multirow{2}{*}{LLaMA2-13B} & W & 7.55 & 0.02 & 5.85 & 0.02 & 3.35 & 0.02 & \cellcolor{red!40}7.87 & 0.02 & 3.43 & 0.02 & 3.15 & 0.02 & 4.03 & 0.02 \\
    & A & 185.16 & 0.40 & 185.16 & 0.40 & 185.16 & 0.40 & 132.78 & 0.12 & 24.16 & 0.27 & 24.16 & 0.27 & \cellcolor{red!40}3.84e5 & 0.14 \\
    \midrule
    \multirow{2}{*}{LLaMA2-70B} & W & 5.53 & 0.01 & 6.75 & 0.02 & 3.22 & 0.01 & \cellcolor{red!40}8.66 & 0.01 & 3.25 & 0.02 & 3.08 & 0.01 & 3.68 & 0.01\\
    & A & 303.04 & 0.28 & 303.04 & 0.28 & 303.04 & 0.28 & 118.70 & 0.09 & 141.58 & 0.25 & 141.58 & 0.25 & \cellcolor{red!40}3.59e5 & 0.14 \\
    \bottomrule
    \end{tabular}}
    \label{tab:base_linear_type_llama2}
    \vspace{-5pt}
\end{table*}

\begin{table}[t]
    \centering
    \caption{The evaluation results of AWQ and SmoothQuant methods on LLaMA2 models on the LAMBADA dataset. ``SQ'' is short for ``SmoothQuant''.}
    \vspace{-5pt}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        % \multirow{3}{*}{LLaMA2} & \multirow{3}{*}{FP16} & \multicolumn{4}{c}{W Quant.} & \multicolumn{2}{c}{WA Quant.} \\
        % \cmidrule(lr){3-6}\cmidrule(lr){7-8}
        % & & \multicolumn{2}{c}{W3} & \multicolumn{2}{c}{W2} & \multicolumn{2}{c}{W4A4} \\ 
        \multirow{3}{*}{LLaMA2} & \multirow{3}{*}{FP16} & \multicolumn{2}{c}{W3} & \multicolumn{2}{c}{W2} & \multicolumn{2}{c}{W4A4} \\ 
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8}
        & & RTN & AWQ & RTN & AWQ  & RTN & SQ \\ 
        \midrule
        7B  & 73.32 & 66.41 & 69.63 &  0.00 &  0.00 &  4.31 & 25.56 \\
        70B & 78.96 & 76.46 & 78.73 & \cellcolor{red!40}16.96 &  \cellcolor{red!80}0.00 & 0.04 & 38.11 \\
        \bottomrule
    \end{tabular}}
    \label{tab:eval_basic_quant_algo}
    \vspace{-15pt}
\end{table}

%% 内容
% 1. Tensor Type的基本规律（数据分析）
% 1.1 模型参数量越大，对KV Cache和Weight量化的容忍度越高。原因是：随着模型增大，权重数据中的绝对数值大小在降低，并且权重数据的峰度在降低（离群数据减少）
% 1.2 模型参数量越大，对Activation量化的容忍度越低。原因是：随着模型增大，Attention和MLP的输入Activation中离群值的绝对数值会增大，峰度也会增大（离群数据增多）
% 
% 2. 模型族的基本规律（数据分析）
% 2.1 OPT族WA更难；
% 2.2 Mixtral对量化更敏感；
% 
% 3. 不同任务的基本规律（数据分析）
% 3.1 （绝对性能）更难的任务上性能损失更大？
% 3.2 （趋势）不同数据集上量化的拐点基本一致？通过数据分析来说明
% 3.3 Recommandation
% 3.4 Case Study：
% 3.4.1 ppl：weight量化更认准一个错误答案
% 3.4.2 ppl：wa、kv量化都比较平均
% 
% 4. 在basic模型上，AWQ和SmoothQuant是否可以显著改善性能拐点。
% 
% Basic 能力专有的问题：
% 1、不同语种有无不同？
% 2、failure cases。
% 
% TODO：
% [x] llama2-7b & 70b smoothquant和AWQ，LAMBADA上。
%       * 已准备好代码；
% [x] 看一下极低位宽下fail的方式，是ppl非常近似还是只固定选一个选项。
%       * 都不是，ppl的差值分布和FP的非常相像。
% [x]llama2-7b、13b、70b lambada & PIQA.
%       * 7b/13b llama2-chat模型实验已启动，70b脚本已准备好。
% [x] 参数量拉平的图、cherry pick一下
% [x] 找人类baseline
\section{Evaluation on Basic NLP Tasks}
\label{sec:eval_basic}

\subsection{Experimental Setups}
% To evaluate the effect of quantization on basic knowledge and abilities of the base LLMs, we employ open-source LLMs without instruction tuning and RLHF for evaluation, including the OPT, BLOOM, LLaMA, Falcon, and Mistral model families.
We evaluate the quantized LLMs on three types of basic NLP tasks: Language Modeling tasks, Natural Language Understanding tasks, and Natural Language Reasoning tasks.
More details can be found in Appendix~\ref{app:basic}.
% Based on the extensive evaluation results, we summarize and analyze the general effects of quantization on various NLP tasks, different LLMs, three tensor types, and SOTA quantization methods.

\subsection{Effects of Quantization on Three Tensor Types}
\label{sec:basic_tensor}
\textbf{The larger the model size, the higher the tolerance for Weight Quantization.}
As shown in Figure~\ref{fig:eval_basic_tensor_lambada} (a), for small models, such as LLaMA2-7B, when quantized to W3, the accuracy significantly degrades.
However, the performance of the W3 quantized LLaMA2-70B exhibits only a marginal decline.
This is because, in the same model family, the Kurtosis of the Weight tensors decreases as the model size grows larger, which means there are fewer outliers in larger LLMs, as illustrated in Table~\ref{tab:eval_basic_statistic}.
In addition, the AbsMax and Std of the larger models are smaller than those of smaller models.
\textbf{Moreover, the KV Cache Quantization exhibits similar phenomena to Weight Quantization.}
In most cases, the larger the model size, the higher the tolerance for KV Cache Quantization.
The AbsMax, Std, and Kurtosis of models with different sizes are similar, and larger models sometimes exhibit similar or slightly decreased Kurtosis compared to smaller models.

\textbf{On the contrary, the larger the model size, the lower the tolerance for Activation Quantization.} 
As shown in Table~\ref{tab:eval_basic_statistic}, the Kurtosis of the Activation tensors ($>$1000) is much larger than that of the Weight and KV Cache tensors ($\sim$10).
This suggests that there are more outliers in the Activation tensors than in the Weight and KV Cache tensors.
Notably, the Kurtosis of the Activation increases significantly with the size of the model, which means more outliers in the Activation tensors of larger LLMs. 

\textbf{Generally speaking, on the majority of tasks, most LLMs can preserve their performance with W4 or KV4 quantization. }
When quantizing LLMs to W3 or KV3, there is a noticeable decline in the performance of small models across all model families. 
Moreover, for W2 or KV2, the majority of models experience a significant performance loss.
\textbf{For Weight-Activation Quantization, the W4A8 LLMs represent the frontier where decent performance can be achieved.}
W4A4 Quantizing will cause the majority of LLMs to experience a complete loss of performance.

In real-world applications with large batch sizes and long texts, one common practice is to quantize both the Weight and KV Cache.
\uline{For tasks with short texts ($<$ 4K), W8KV4 is nearly lossless for many tasks ($<$ 2\% performance loss).
For tasks with long texts ($\geq$ 4K), W8KV8 may be a better choice ($<$ 2\% performance loss).}
More details are in Appendix~\ref{app:basic_tensor}.

In addition, as shown in Table~\ref{tab:base_linear_type_llama2}, we find that different linear layers have distinct Kurtosis.
For instance, within the LLaMA2 family, the kurtosis of the activation in down projection layers in FFN is notably higher compared to other layers, and the kurtosis of the weight in out projection layers in Attention is slightly higher than that of the other layers.
A similar phenomenon also appears in other LLM families, such as OPT and Mamba in Table~\ref{tab:base_linear_type_opt} and Table~\ref{tab:base_linear_type_mamba}.
\textbf{This phenomenon suggests that employing different bit-width and scaling schemes for different tensors might be promising to balance the hardware efficiency and performance as discussed in Appendix~\ref{app:basic_statistic}.}

\subsection{Effects of Quantization on Different LLMs}
\label{sec:basic_llms}
% \textbf{For the majority of LLMs, the performance order of the Weight-only, Weight-Activation, and KV Cache quantized LLMs is generally consistent with that of the FP16 LLMs when the bit-width is higher than W4, W4A8, and KV4.} 
\textbf{The relative rankings of quantized LLMs are generally consistent with those of the FP16 LLMs when the bit-width is higher than W4, W4A8, and KV4.} 
Details can be found in Appendix~\ref{app:basic_llms}.

% \textbf{Different from increasing the width and depth, 
\textbf{Leveraging the Mixture-of-Experts (MoE) technique to increase the model size may not necessarily enhance the model's tolerance to quantization.}
As depicted in Figure~\ref{fig:eval_basic_tensor_lambada}, the performance of the FP16 Mixtral-8x7B MoE model is similar to LLaMA2-70B.
However, Mixtral-8x7B is more sensitive to Weight-only and KV Cache Quantization than LLaMA2-70B.
%As shown in Figure~\ref{fig:eval_basic_tensor_lambada} (a, c), after the W3 or KV3 quantization, the performance loss of Mixtral-8x7B is notably higher than that of LLaMA2-70B.
Instead, the sensitivity of Mixtral-8x7B to quantization is closer to that of the smaller LLaMA2-7B and Mistral-7B from the same model family. 


% \begin{table}[t]
%     \centering
%     \caption{The PPL statistical results for the W8A8 Mistral-7B model on multiple-choice task RACE.}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{ccccccccc}
%     \toprule
%     \multirow{2}{*}{Bit-width} & \multicolumn{2}{c}{C1}  & \multicolumn{2}{c}{C2} & \multicolumn{2}{c}{C3} & \multicolumn{2}{c}{C4}  \\
%     \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
%     & PPL & Std & PPL & Std & PPL & Std & PPL & Std \\
%     \midrule
%     FP16    & \cellcolor{red!20}1.996 & 0.0016 & \cellcolor{red!20}2.020 & 0.0011 & \cellcolor{red!20}2.021 & 0.0013 & \cellcolor{red!20}2.021 & 0.0011 \\
%     W8A8      & \cellcolor{red!40}2.011 & 0.0015 & \cellcolor{red!40}2.035 & 0.0010 & \cellcolor{red!40}2.036 & 0.0012 & \cellcolor{red!40}2.035 & 0.0010 \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:basic_ppl_tasks}
%     \vspace{-15pt}
% \end{table}

%\vspace{-10pt}
\subsection{Effects of Quantization on Different Tasks}
\label{sec:basic_tasks}

%\textbf{The quantized LLMs do not yield distinct impacts on tasks organized in different languages.}
\textbf{We do not observe significantly different impacts of quantization across different languages.}
We evaluate various quantized LLMs on the CHID and Winogrande datasets, which are cloze tasks presented in Chinese and English, respectively.
Despite the diverse performance of different LLMs on these tasks, the trend of performance loss caused by quantization is similar.
Moreover, evaluations on CEval and MMLU in Appendix~\ref{app:emergent_results} show consistent findings.

% \textbf{Multi-choice accuracy sometimes cannot accurately reflect the performance.}
% For multiple-choice tasks, we concatenate each answer candidate with the question to form multiple sentences (see Appendix~\ref{app:basic_metrics}).
% Then, we compute the perplexity (PPL) of each sentence and choose the sentence with the lowest PPL as the answer. 
% We observe that in some cases, quantization even brings notable accuracy gain.
% For example, the accuracy of Mistral-7B on the RACE dataset increases by $3.5\%$ after W8A8 quantization.
% We look into this unexpected phenomenon as follows. We categorize multiple-choice questions into four classes, as presented in Table~\ref{tab:basic_ppl_tasks}.
% C1 and C4 denote questions for which both the FP16 and W3 Mistral-7B answer correctly and incorrectly, respectively.
% C2 denotes questions answered correctly before quantization but incorrectly after quantization, while C3 is the opposite.
% We compute the average PPL for the correct answers and the average standard deviation (Std) of PPL within each of the four categories.
% %We compute the average perplexity (PPL) for the correct answers across all questions and the average standard deviation (Std) of the PPL for each of the four options.
% We observe that
% (1) The average PPL increases after quantization, indicating a decline in performance for quantized LLMs. 
% (2) The average Std in C2 and C3 is notably smaller than that in C1 and C4.
% This suggests that questions in C2 and C3 are instances where the model exhibits high uncertainty. Consequently, it is possible for the quantized model to guess the correct answer, resulting in the phenomenon that quantization brings accuracy gain.


For the majority of tasks and LLMs, we summarize the recommendations for the quantization bit-width:
\uline{(1) As discussed in Section~\ref{sec:basic_tensor}, for most LLMs and tasks, W4, W4A8, and KV4 quantization has negligible performance loss ($<$ 2\%), as shown in Table~\ref{tab:intro_knowledge}.}
(2) Furthermore, under a specific memory budget, we may use the larger model with W3 quantization for most tasks.
For example, in Figure~\ref{fig:eval_basic_tasks} (a), the performance of W3 LLaMA-70B is better than FP16 LLaMA2-13B on the RACE task with 27GB memory.
(3) When the phenomenon of ``performance saturation'' occurs, i.e., the performance no longer increases as the model grows larger (as observed with Bloomz-3B and Bloomz-7B1 in Figure~\ref{fig:eval_basic_tasks} (b)), a better choice may be to use a smaller model with a higher bit-width.


% \subsection{Effects of Quantization methods}
% \label{sec:basic_methods}
% \textbf{Restoring performance to a level similar to the FP16 LLMs is challenging with SOTA quantization methods when using extremely low bit-width, such as W2 or W4A4.}
% As shown in Table~\ref{tab:eval_basic_quant_algo}, we observe that for the W3 quantization, AWQ can improve the performance of quantized LLMs.
% Moreover, the larger the model, the closer the performance is to the FP16 baseline.
% However, in the case of W2 quantization, where quantized LLMs lose their abilities entirely, AWQ cannot restore the corrupted performances.
% Similar results are also observed with Weight-Activation Quantization. 
% While SmoothQuant can partially recover the performance for W4A4 quantization, the performance remains significantly lower than the FP16 baseline.
% The conclusions are applicable to other tasks as well, and additional details can be found in our Appendix.
% Specifically, the results for emergent abilities are shown in Table~\ref{tab:emergent_quant_algo}, dialogue results can be found in Table~\ref{tab:dialogue}, and long-context evaluations are depicted in Figure~\ref{fig:app_longeval_awq}.


%We recommend applying the SOTA quantization methods when the performance is not significantly affected. 
%However,
To make extremely low bit-width quantization work, such as W2 and W4A4, further research on quantization schemes or quantization-aware training (QAT) methods~\cite{llmqat} is needed.
For KV2, the recently proposed window-based quantization method~\cite{kivi} shows promise of being achievable.


==> ICML24/Sections/eval_dialogue.tex <==
\begin{figure*}[t]
    % \vspace{-10pt}
    \centering
    \subfigure[W-only Quant.]{
        \centering
        \includegraphics[width=0.3\linewidth]{Figures/long/LongEval_w_Length.pdf}
    }
    \subfigure[WA Quant.]{
        \centering
        \includegraphics[width=0.3\linewidth]{Figures/long/LongEval_wa_Length.pdf}
    }
    \centering
    \subfigure[KV Cache Quant.]{
        \centering
        \includegraphics[width=0.3\linewidth]{Figures/long/LongEval_kv_Length.pdf}
    }
    \vspace{-5pt}
    \caption{The effect of quantization on effective context length. %(a, b, c) and context position (d, e, f). 
    The blue and red lines represent the Mixtral-8x7B (32K) and Vicuna-7B (16K) models, respectively. }
    \label{fig:eval_long-longchat}
\end{figure*}

\begin{table*}[]
    \centering
    % \vspace{-10pt}
    \caption{The effect of quantization on multi-turn dialogue benchmark MT-bench. ``SQ'' is short for ``SmoothQuant''. }
    \vspace{-5pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccccccccccc}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Turn} & \multirow{2}{*}{FP16} & \multicolumn{4}{c}{W Quant.} & \multicolumn{4}{c}{WA Quant.} & \multicolumn{3}{c}{KV Cache Quant.} \\
        \cmidrule(lr){4-7}\cmidrule(lr){8-11}\cmidrule(lr){12-14}
         & & & W8 & W4 & W3 & W3(AWQ) & W8A8 & W4A8 & W4A4 & W4A4(SQ) & KV8 & KV4 & KV3 \\ 
        \midrule
        \multirow{2}{*}{LLaMA2-13B-chat} & 1 & 5.72 & 5.95 & 5.74 & 5.38 & 5.71 & 5.83 & 5.88 & 1.00 & 2.34 & 5.84 & 5.86 & \cellcolor{red!40}5.53 \\
        & 2 & 5.05 & 5.31 & 4.65 & 4.26 & 4.19 & 5.12 & 4.97 & 1.00 & 1.51 & 5.04 & \cellcolor{red!40}4.38 & \cellcolor{red!80}3.85 \\ 
        \midrule
        \multirow{2}{*}{LLaMA2-70B-chat} & 1 & 6.26 & 6.49 & 5.91 & 5.86 & 6.38 & 6.17 & 6.11 & 1.00 & 2.09 & 6.41 & 6.30 & 6.25 \\
        & 2 & 5.99 & 5.83 & 5.55 & 5.12 & 5.44 & 5.86 & 5.86 & 1.00 & 1.56 & 5.91 & 6.03 & 5.66 \\ 
        \bottomrule
    \end{tabular}}
    \label{tab:eval_dialogue}
    % \vspace{-10pt}
\end{table*}

% \vspace{-10pt}
\section{Evaluation on Dialogue Tasks}
\label{sec:eval_dia}

\subsection{Experimental Setups}
We evaluate the dialogue quality of quantized LLMs on the MT-bench~\cite{MT-bench}, a two-turn dialogue benchmark.
We use GPT-4-0613 to generate single-answer grading (GPT-4 score) for each generated dialogue, ranging from 1 to 10.
More details can be found in Appendix~\ref{app:dia_metrics}.

\vspace{-5pt}
\subsection{Experimental Results}
\textbf{The tolerance of dialogue abilities to KV Cache Quantization is higher than Weight Quantization for most LLMs.}
\uline{Most LLM families can be quantized to W8, W8A8, and KV4 without significant loss of GPT-4 score ($<2\%$), as shown in Table~\ref{tab:intro_knowledge}.}
As shown in Table~\ref{tab:eval_dialogue}, 
W4 quantization causes a significant loss of the GPT-4 score by $>0.3$ on both LLaMA2-13B and LLaMA2-70B.
In terms of the concrete failure patterns, we observe that (1) With W3 and KV3 quantization, most LLMs begin to repeat some sentences.
(2) With W2, KV2, and W4A4, most LLMs lose their dialogue ability and generate meaningless symbols or repeat some words.
(3) Only a few LLMs, such as ChatGLM3-6B, Falcon-40B, and Falcon-180B, can still generate coherent sentences under KV2 quantization, although most sentences lack meaningful content.
More details are shown in Appendix~\ref{app:dia_case}.
% It is worth noting that for the Mamba family, we evaluate an unofficial mamba-2.8B-chat model~\cite{mambachat} only for reference.
% The GPT-4 score of FP16 Mamba-2.8B-chat is around 1, showing a significant gap compared to Gemma-2B and StableLM-3B models with similar parameter sizes.
% Therefore, further analysis of its sensitivity to quantization may not be meaningful now.

Additionally, it is noteworthy that the FP16 performance of some recent small models, such as StableLM-3B, is on par with that of Falcon-40B.
However, the sensitivity of StableLM-3B to quantization is more similar to that of the smaller Falcon-7B, as shown in Table~\ref{tab:dialogue}.
\textbf{This might suggest that small models with enhanced FP16 performances might not necessarily have a higher tolerance to quantization.}
% As depicted in Figure~\ref{fig:eval_basic_tensor_lambada}, the performance of the FP16 Mixtral-8x7B MoE model is similar to LLaMA2-70B.
% However, Mixtral-8x7B is more sensitive to Weight-only and KV Cache Quantization than LLaMA2-70B.
%As shown in Figure~\ref{fig:eval_basic_tensor_lambada} (a, c), after the W3 or KV3 quantization, the performance loss of Mixtral-8x7B is notably higher than that of LLaMA2-70B.
% Instead, the sensitivity of Mixtral-8x7B to quantization is closer to that of the smaller LLaMA2-7B and Mistral-7B from the same model family. 

%In addition, as the quantization bit-width decreases, there are noticeable patterns of degradation in dialogue ability.

%In the dialogue task, we observe that smaller models (StableLM-3B) are more sensitive to Weight-only and KV Cache Quantization while being less sensitive to Weight-Activation Quantization, as illustrated in Table~\ref{tab:dialogue} in Appendix~\ref{app:dia_case}.

% \textbf{Do different tensor types have distinct effects after quantization?}
% \textit{The models demonstrate similar robustness in quantization for weight and KV Cache.}
% The majority of models exhibit similar performance when quantizing weight and KV Cache. 
% When quantized to 4-bit, both weight and KV Cache quantization maintain conversation performance. 
% When quantized to 3-bit, both quantization methods result in slight conversation performance loss. 
% When quantized to 2-bit, both quantization methods lead to the model almost completely losing its conversational ability. 
% Although there may be slight differences in the robustness of some models to weight and KV Cache quantization, these differences are typically small, and we do not observe a clear relationship between these differences and model family or model size.

In MT-Bench, the second-turn dialogue consistently yields lower GPT-4 scores compared to the first turn.
\textbf{Nevertheless, the effects of quantization do not show significant differences for two-turn dialogues in most LLMs.}
An exception is that when quantizing the KV Cache from KV8 to KV3, LLaMA2-13B experiences a significant drop in the GPT-4 score of the second-turn dialogue by 1.19, while the GPT-4 score of the first-turn dialogue only decreases by 0.31, as shown in Table~\ref{tab:eval_dialogue}.

\textbf{For the dialogue task, achieving a performance level similar to FP16 LLMs remains challenging when using extremely low bit-width, such as W2 or W4A4 with AWQ~\cite{AWQ} or SmoothQuant~\cite{smoothquant}.}
In the case of Weight-only Quantization with AWQ, certain models, such as Falcon-7B and Falcon-40B, exhibit slight improvements in W2 quantization.
Specifically, they can generate some coherent yet meaningless sentences.
Regarding Weight-Activation Quantization, SmoothQuant can recover dialogue ability for some LLMs when quantized to W4A4.
As illustrated in Table\ref{tab:eval_dialogue}, quantizing to W4A4 with SmoothQuant results in higher GPT-4 scores for LLaMA2-13B and LLaMA2-70B, enabling them to generate meaningful responses, especially in the first-turn dialogue.

In the future, it is worth investigating the impact of quantization on dialogues with more than two turns. 
Whether quantization will have a more significant effect after several turns of dialogue remains unknown.

==> ICML24/Sections/eval_emergent.tex <==
\begin{figure*}[t]
% \vspace{-10pt}
    \centering
    \subfigure[W-only Quant. on LLaMA2-7B]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/emergent/LLaMA2-7B_w.pdf}
    }%
    \centering
    \subfigure[WA Quant. on LLaMA2-7B]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/emergent/LLaMA2-7B_wa.pdf}
    }%
    \centering
    \subfigure[KV Cache Quant. on LLaMA2-7B]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/emergent/LLaMA2-7B_kv.pdf}
    }%
    \vspace{-5pt}
    \caption{The effect of quantization on four emergent abilities. We normalize the performance of quantized LLMs based on the performance of FP16 LLMs. ``ICL'', ``C-MR'', ``M-MR'', ``IF'', ``SC'' are short for ``In-Context Learning'', ``Commonsense Multi-Step Reasoning'', ``Mathematical Multi-Step Reasoning'', ``Instruction-Following'', and ``Self-Calibration''.}
    \label{fig:eval_icl_inst}
    % \vspace{-5pt}
\end{figure*}



% 特有的现象和知识：
% 1. 模型层面：
% 1.1 Mistral和其他模型基本是反的。下降幅度更大
% 1.2 LLaMA2模型的KV cache普遍可以到2-bit

% 2. 任务层面：
% 2.1 能力损失的顺序？没有明显的顺序
% 2.2 In-context learning中增加样本到底会不会进一步提升性能？
% 2.3 AWQ、Smoothquant有没有能够有效将拐点推到更低位宽？

% TODO：
% 1. Self-calib有什么新现象
% 2. AWQ、Smoothquant在GSM8K。
% 3. In-context learning中增加样本
% 4. Case Study：2-bit量化之后的现象。到底是推理链条能生成但是结果都错了，还是干脆都崩了。
% 5. 找人类baseline。


\vspace{-10pt}
\section{Evaluation on Emergent Abilities}
\label{sec:eval_emergent}

\subsection{Experimental Setups}
% To evaluate the effect of quantization on the emergent abilities shown in LLMs, we employ open-source instruction-tuned LLMs for evaluation, including the LLaMA, Falcon, ChatGLM, and Mistral model families.
We evaluate four emergent abilities~\cite{emergent}, including In-Context Learning, Instruction-Following, Multi-Step Reasoning, and Self-Calibration. More details about the task formulation are in Appendix~\ref{app:emergent_metrics}.


% \vspace{-10pt}
\subsection{Experimental Results}

\textbf{Among four emergent abilities, the tolerance of Multi-Step Reasoning and Self-Calibration abilities to quantization is notably lower than that of the Instruction-Following and In-Context Learning abilities, especially for small LLMs.}
% We show the performance of the quantized LLaMA2-7B model on the four different abilities in Figure~\ref{fig:eval_icl_inst}. 
As shown in Figure~\ref{fig:eval_icl_inst}, the W3 or KV3 LLaMA2-7B exhibits a near-complete loss of its Self-Calibration ability. This loss is significantly larger than those of Instruction-Following and In-Context Learning abilities.
Among the two types of Multi-Step Reasoning tasks, we find that the mathematical task is much more sensitive than the common-sense task.
Mathematical Multi-Step Reasoning exhibits a tolerance similar to Self-Calibration,  while Common-sense Multi-Step Reasoning shows a tolerance similar to In-Context Learning and Instruction-Following.
The Gemma model family is an exception, with its In-Context Learning ability showing a lower tolerance to quantization compared to its Mathematical Multi-Step Reasoning ability, as shown in Figure~\ref{fig:app_emergent_Gemma_2B} and Figure~\ref{fig:app_emergent_Gemma_7B}.

% Furthermore, for the sensitive Mathematical Multi-Step Reasoning ability, we categorized and counted the various errors produced by LLaMA2-70B after quantization, as shown in Figure~\ref{fig:emergent_gsm8k_failure_type}.
Furthermore, for the sensitive Mathematical Multi-Step Reasoning ability, we categorized the quantization errors into four types: incorrect logic, calculation error, copy mistake, and condition missing, as shown in Appendix~\ref{app:emergent_results}.
We also summarize the proportion of each error type for LLaMA2-70B after quantization, as shown in Figure~\ref{fig:emergent_gsm8k_failure_type}.
For Weight-only quantization and KV Cache quantization, there are fewer errors at 4-bit, but the model fails at 2-bit, so we summarize the results for W3 and KV3.
Similarly, for Weight-Activation quantization, there is almost no loss at W8A8, but the model fails at W4A4, so we summarize the results for W4A8.
\textbf{The evaluation results show that the major error type is incorrect logic, accounting for around 50\%, much higher than the second most common error, calculation error, at around 20\%.}
How to ensure that low-bit LLMs maintain good problem-solving logic should be the main focus of future quantization methods.



\uline{For the evaluated benchmarks, for smaller LLMs ($<13$B), W8, W8A8, or KV8 is more suitable to maintain Multi-Step Reasoning and Self-Calibration abilities within 2\% performance loss.
For larger models ($\geq13$B), W4, W4A8, or KV4 is enough to maintain all four emergent abilities within 2\% performance loss.}
% In addition, for most LLMs,  does not lead to significant performance loss, but W4A4 results in a complete loss of emergent abilities for all models.
More experimental results can be found in Appendix~\ref{app:emergent_results}.
% Note that for the Mamba family, since there are no official instruction-tuned models,  we only evaluate their In-Context Learning ability. The phenomenon is similar to other model families, as shown in Table~\ref{tab:emergent_quant_shots_mamba}.

% \textbf{Both AWQ and SmoothQuant can benefit the emergent abilities, as described in Sec.\ref{sec:basic_methods}.}
% We evaluate AWQ and SmoothQuant on the hard GSM8K datasets.
% For W3 quantization, AWQ can truly improve the performance, and the larger the model, the greater the performance improvement.
% For W2 and W4A4 quantization, AWQ and SmoothQuant both fail to improve the performance.

% \ul{In summary, for the hard self-calibration and multi-step reasoning abilities, especially the mathematical tasks, we recommend applying W8, W8A8, and KV8. For other emergent abilities, W4, W4A8, and KV4 are acceptable.}
% \ul{In summary, for the hard self-calibration and multi-step reasoning abilities, especially the mathematical tasks.}
% \todo{Detail analysis}

==> ICML24/Sections/eval_long.tex <==
\section{Evaluation on Long-Context Tasks}
\label{sec:eval_long}

\subsection{Experimental Setups}
We evaluate the quantized long-context LLMs on a key-value retrieval task~\cite{longchat} with a context length of up to 16K tokens and a multi-document question-answering task~\cite{lost_in_the_middle} with a context length of up to 6K tokens.
Additional details can be found in Appendix~\ref{app:long_data}.

\subsection{Experimental Results}
\label{sec:eval_long_result}
\textbf{Long texts ($\geq$4k) are more sensitive to Weight-only and KV Cache Quantization than short texts ($<$4k).}
For Weight-only Quantization, the performance loss in long texts is significantly larger than that in short texts.
Figure~\ref{fig:eval_long-longchat} (a) illustrates that when quantized to W3, both the Mixtral-8x7B and Vicuna-7B models experience a more significant accuracy loss on longer texts. 
Similar results are observed for other LLMs in Appendix~\ref{app:long_longeval}. 
As for Weight-Activation Quantization, the quantized model does not show larger performance degradation in long texts than in short texts, as shown in Figure~\ref{fig:eval_long-longchat} (b). 

\textbf{For long-context tasks ($\geq$4k), most LLMs are more sensitive to KV Cache Quantization than Weight-only and Weight-Activation Quantization.}
With the same bit-width, the performance of LLMs with KV Cache Quantization is notably lower than that of Weight-only Quantization, as shown in Figure~\ref{fig:eval_long-longchat} (a, c).
Within the LongChat (LLaMA-based) family, even KV8 quantization will cause notable performance degradation on long texts.
For the Vicuna (LLaMA2-based) and ChatGLM family (32K), KV8 quantization is almost lossless, and the performance degradation on long texts occurs when using KV4.
The Mistral family shows the highest tolerance to KV Cache Quantization, which is different from short texts. 
KV4 is still lossless for the Mistral family.

\uline{On LongEval and Multi-Doc QA benchmarks, within 2\% accuracy loss, most LLMs can be quantized to W4, W4A8, or KV4 for short texts ($<$4k), and W4, W4A8, or KV8 for long texts ($\geq$4k), as illustrated in Table~\ref{tab:intro_knowledge}.}



% \uline{In summary, for most LLMs, we recommend applying W4, W4A8 and KV8 for long-context tasks.
% Besides, there is limited research on quantization methods specifically tailored for long-context tasks, and it is deserving of attention in the future.}


==> ICML24/Sections/eval_trust.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[W-only Quant. on Moral]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/trust/commonsense_w_Bit-width.pdf}
    }%
    % \subfigure[Weight-only Quant. on Virtue]{
    %     \centering
    %     \includegraphics[width=0.33\linewidth]{Figures/trust/virtue_w_Bit-width.pdf}
    % }%
    \subfigure[Case 1: W-only Quant.]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/trust/ethics_w_answer.pdf}
    }%
    % \centering
    % \subfigure[KV Cache Quant. on Moral]{
    %     \centering
    %     \includegraphics[width=0.33\linewidth]{Figures/trust/commonsense_kv_Bit-width.pdf}
    % }%
    % \subfigure[KV Cache Quant. on Virtue]{
    %     \centering
    %     \includegraphics[width=0.33\linewidth]{Figures/trust/virtue_kv_Bit-width.pdf}
    % }%
    \subfigure[Case 2: KV Cache Quant.]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/trust/ethics_kv_answer.pdf}
    }%
    % \vspace{-10pt}
    \caption{The effect of quantization on the Ethics Benchmark.}
    \label{fig:eval_trust-ethic}
\end{figure*}


\begin{figure*}[t]
    % \centering
    % \subfigure[Case 1: FP16 (Layer 14)]{
    %     \centering
    %     \includegraphics[height=0.22\linewidth]{Figures/trust/vis/fp16-w.pdf}
    % }
    % \subfigure[Case 1: W3 (Layer 14)]{
    %     \centering
    %     \includegraphics[height=0.22\linewidth]{Figures/trust/vis/w3-w.pdf}
    % }
    % \subfigure[Case 2: FP16 (Layer 6)]{
    %     \centering
    %     \includegraphics[height=0.22\linewidth]{Figures/trust/vis/fp16-kv.pdf}
    % }
    % \subfigure[Case 2: KV3 (Layer 6)]{
    %     \centering
    %     \includegraphics[height=0.22\linewidth]{Figures/trust/vis/kv3-kv.pdf}
    % }
    \centering
    \includegraphics[width=\linewidth]{Figures/trust/ethics_attention.pdf}
    % \vspace{-20pt}
    \caption{Changes in the attention maps of Layer 14 in the quantized LLaMA2-7B on the Ethics Benchmark.}
    \label{fig:eval_trust-ethic-attention}
\end{figure*}


\section{Evaluation on Trustworthiness}
\label{sec:eval_trust}

\subsection{Experimental Setups}
We evaluate three types of trustworthiness tasks of the quantized LLMs, including Ethics,  Hallucination, and Adversarial Robustness tasks.
Overall, the phenomena of hallucination and adversarial tasks are similar to the basic NLP tasks, as discussed in Sec.~\ref{sec:eval_basic}.
We only discuss the different phenomena observed in the Ethics tasks.
Additional results can be found in Appendix~\ref{app:trust}.

\subsection{Experimental Results}
\textbf{Different tensor types have distinct effects after quantization, especially the Weight and KV Cache tensors for small LLMs within 7B.} 
We analyze the generation results of the Weight-only quantized LLMs shown in Figure~\ref{fig:eval_trust-ethic} (b).
The FP16 LLM refrains from answering some ethical questions, but for W3, the model breaks this limitation and begins to provide informative answers.
To this end, the performance will increase, as shown in Figure~\ref{fig:eval_trust-ethic} (a). 
After applying AWQ, there is a slight decrease in accuracy for the LLaMA2-7B model on the moral task because the LLM stops answering some sensitive questions, as shown in Figure~\ref{fig:eval_trust-ethic} (a). 
In contrast, after quantizing the KV Cache of LLMs, they start to refrain from answering more questions, and the model's outputs become more restricted, as shown in Figure~\ref{fig:eval_trust-ethic} (c).
Note that this phenomenon only appears in small models ($<$ 7B). For large models, the lower the bit-width, the lower the performance ($\geq$ 7B). 
% Moreover, compared to smaller models, large models refrain from answering only a few questions and provide accurate answers to most queries.

To delve deeper into the aforementioned phenomenon, we examine how quantization affects the attention map of LLaMA2-7B, illustrated in Figure~\ref{fig:eval_trust-ethic-attention}.
We average the attention map of each head in one layer to get the overall attention map for analysis. 
For W3 quantization, we notice that after quantization, the model will pay more attention to the original questions, which is why the model will generate certain answers, as shown in Figure~\ref{fig:eval_trust-ethic-attention} (a) and (b).
Conversely, with KV3 quantization, we observe a decrease in attention toward the original question after quantization, leading to less informative answers, as shown in Figure~\ref{fig:eval_trust-ethic-attention} (c) and (d).


\uline{As illustrated in Table~\ref{tab:intro_knowledge}, in our evaluation, within 2\% accuracy loss, for smaller LLMs ($<$ 7B), W8, W8A8, or KV8 is recommended.
For larger LLMs ($\geq$ 7B), W4, W4A8, or KV4 is recommended.}
% However, in fact, the generation results of the quantized LLaMA2-7B are closer to that of the original model.

% \ul{In the future, it is worthwhile to conduct in-depth research and propose more datasets and metrics that more accurately reflect the trustworthiness of models, especially in terms of ethics and privacy. 
% Additionally, applying quantization to enhance trustworthiness is also a promising direction for research.}



==> ICML24/Sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

Nowadays, Large Language Models (LLMs) have showcased remarkable performance in a variety of tasks, including natural language understanding and generation. 
Notably, the advent of LLMs has given rise to several interesting and valuable applications, such as ChatGPT~\cite{openai2023gpt4} and Copilot~\cite{copilot}.
However, the efficient deployment of LLMs poses a substantial challenge due to their considerable memory consumption and computational overhead. 

%Diverging from traditional Convolutional Neural Network (CNN) models,
The LLM inference process encompasses two stages: the prefill stage and the decoding stage.
The prefill stage is primarily compute-bound, while the decoding stage, characterized by small batch sizes, is generally memory-bound. 
Furthermore, when processing tasks involving long texts or large batch sizes, the memory overhead associated with the Key-Value Cache (KV Cache) surpasses that of the Weights.
% Furthermore, in the processing of tasks involving long texts or large batch sizes, the memory overhead associated with the Key-Value Cache (KV Cache) surpasses that of the weights.

An effective approach to address the aforementioned challenge is post-training quantization (PTQ)~\cite{wan2023efficient,zhou2024survey}.
PTQ methods aid in the reduction of the memory consumption of Weights, Activations, and KV Caches by using the low-precision values with fewer bits instead of the high-precision values.
(1) The Weight-only Quantization methods prove effective in accelerating the memory-bounded General Matrix-Vector Multiply (GEMV) operators in the decoding stage~\cite{AWQ,LUTGEMM,GPTQ,squeezellm,owq}.
(2) The Weight-Activation Quantization methods enable the utilization of low-precision Tensor Cores in GPUs to mitigate the compute-bounded General Matrix Multiply (GEMM) operators in the prefill stage~\cite{smoothquant, outlier,llmint8,zeroquant,rptq}.
(3) The KV Cache Quantization methods are helpful in alleviating memory overhead when handling long texts or large batch sizes~\cite{FlexGen}.


\begin{table*}[t]
    \centering
    \caption{The summary of the discovered key knowledge.}
    \vspace{-5pt}
    \begin{tabular}{cp{13.5cm}}
    \toprule
    Knowledge Level &  \multicolumn{1}{c}{Key Knowledge} \\
    \midrule

    \multirow{4}{*}{Tensor-level} & \textbf{1. Tensor type (Sec.~\ref{sec:basic_tensor})}: The larger the model, the higher the tolerance for Weight-only and KV Cache Quantization, while the tolerance for Activation Quantization is lower. \\
    ~ & \textbf{2. Tensor position (Sec.~\ref{sec:basic_tensor})}: The sensitivity to quantization varies significantly across different tensor positions due to their distinct data distributions.\\
    
    \midrule
    
    \multirow{4}{*}{Model-level} & \textbf{1. (Sec.~\ref{sec:basic_llms})} The relative rankings of quantized LLMs are generally consistent with those of the FP16 LLMs when the bit-width is higher than W4, W4A8, and KV4. \\
    ~ & \textbf{2. (Sec.~\ref{sec:basic_llms})} Leveraging MoE to increase the model size can improve the model's performance but may not improve the tolerance to quantization.\\

    \midrule
    
    \multirow{7}{*}{Task-level} & \textbf{1. Emergent abilities (Sec.~\ref{sec:eval_emergent})}: The tolerance of Multi-Step Reasoning and Self-Calibration to quantization is lower than that of Instruction-Following and In-Context Learning abilities. \\
    ~ & \textbf{2. Dialogue tasks (Sec.~\ref{sec:eval_dia})}: As the bit-width decreases, sentence-level repetition occurs first, followed by token-level repetition, and token-level randomness. \\
    ~ & \textbf{3. Long-Context tasks (Sec.~\ref{sec:eval_long})}: The longer the text, the larger the performance loss caused by Weight and KV Cache quantization. Most LLMs are more sensitive to KV Cache Quantization than Weight-only and Weight-Activation Quantization.\\

    \midrule

    ~ & \textbf{1. Basic NLP tasks (Sec.~\ref{sec:eval_basic})}: W4, W4A8, KV4, W8KV4. \\
    ~ & \textbf{2. Emergent (Sec.~\ref{sec:eval_emergent})}: W8, W8A8, KV8 ($<$ 13B); W4, W4A8, KV4 ($\geq$ 13B). \\
    Bit-width & \textbf{3. Trustworthiness (Sec.~\ref{sec:eval_trust})}: W8, W8A8, KV8 ($<$ 7B); W4, W4A8, KV4 ($\geq$ 7B). \\
    Recommendation & \textbf{4. Dialogue (Sec.~\ref{sec:eval_dia})}: W8, W8A8, KV4.\\
    ~ & \textbf{5. Long-Context (Sec.~\ref{sec:eval_long})}: W4, W4A8, KV4 (token $<$ 4K); W4, W4A8, KV8 (token $\geq$ 4K).\\
    ~ & \textit{(Note: Within \textbf{2\%} accuracy loss on the evaluated tasks. The recommended quantization bit-width may not generalize to other LLMs or tasks)} \\
    \bottomrule
    \end{tabular}
    \label{tab:intro_knowledge}
    \vspace{-10pt}
\end{table*}

% (2) 不同大小的模型，用不同batch size给不同长度推理，不同stage，在不同硬件平台，efficiency bottleneck不同。 => 不同场景需要不同类量化方法 different types of quantization methods (e.g., ). 
% As a lossy compression technique, 量化方法的design choice很多， (e.g,., 格式，位宽，参数决定方式等等）会影响算法性能。
% (1) 与传统模型不同的是，通用大语言模型会被用在vastly different tasks。不同task对量化敏感性可能非常不同，已有量化方法工作在部分任务上做了验证，然而这些方法是否在其它常用任务上也能保持良好性能是不得而知的。practitioner需要一些经验知识来指导量化方法选型。 ....
%A comprehensive evaluation of the quantized LLMs' performance remains to be undertaken.
% At the efficiency level, deploying LLMs involves considerations for different scenarios, including varying hardware, batch sizes, and text lengths, leading to diverse design choices for quantization.
% As a lossy compression technique, different design choices have distinct effects on real-world tasks.
% At the performance level, unlike traditional models, LLMs can be generally used in vastly different tasks. 
% The sensitivity of quantization effects may vary across diverse tasks. 

As described above, to optimize LLMs for efficiency in various scenarios, such as differing model sizes, batch sizes, text lengths, and hardware, diverse design choices for quantization are needed. Since quantization is a lossy compression technique, alterations in design choices for efficiency considerations will also yield distinct impacts on task performances. 
Especially considering that the current LLMs are serving as general solvers applicable to vastly different tasks, understanding the implications of diverse quantization choices on task performance becomes a crucial question in the application of quantization methods. 

To this end, recently, \citet{q_tensor} study the effect of quantization on Weight and Activation in language modeling tasks without considering the KV Cache Quantization.
\citet{q_emergent} only focus on evaluating three emergent abilities of quantized LLMs without considering important tasks such as trustworthiness, dialogue, and long-context tasks.
These existing efforts, while valuable, have not presented a comprehensive understanding of whether diverse quantization methods can be applied across a broad spectrum of models while preserving task performance across a wide range of tasks.

%Despite these efforts, i

%Practical knowledge is important to guide the selection of appropriate quantization methods.





%While the effectiveness of PTQ has been claimed in many studies, 
% design choice
%现在已经有很多针对不同模型、不同任务、不同场景设计




% 不同任务 task (不同长度；不同任务)
% 不同能力 ability (主要是几类emergent ability)
% 不同模型族 model family，不同模型大小 model size
% 不同量化Tensor类型, tensor type
% 不同量化方法 method (格式 format FP/非均匀; 参数 parameter包括bitwidth/granurity/scale/zeropoint; 值 rep/rounding/training)




In this paper, we make a comprehensive evaluation of quantized LLMs to reveal the status quo across four dimensions:
\textbf{(1) Effect of quantization on various NLP tasks}: 
Existing quantization methods mainly evaluate the quantized models on zero-shot understanding tasks and language modeling tasks. 
Whether quantized LLMs still perform well on other essential tasks, such as dialogue, long-context processing, and trustworthiness tasks, remains unknown.
% In addition, do different tasks exhibit varying tolerances to quantization?
\textbf{(2) Effect of quantization on various LLMs}: After quantization, is there any consistent trend in the performance degradation of the LLMs from different model families and different model sizes?
\textbf{(3) Effect of quantizing different tensor types}: What are the effects on LLMs' performance when quantizing Weight, Activation, and KV Cache tensors? 
Existing methods mainly focus on quantizing Weight and Activation, while detailed performance evaluation of KV Cache Quantization is lacking.
\textbf{(4) Effects of different quantization methods}: Can the commonly employed SOTA quantization methods, such as AWQ~\cite{AWQ} and SmoothQuant~\cite{smoothquant}, effectively recover the performance loss? 

Specifically, %in order to evaluate the effect on different model families and model sizes, 
we evaluate the OOPT, LLaMA2, Falcon, Bloomz, Mistral, ChatGLM, Vicuna, LongChat, StableLM, Gemma, and Mamba model families, spanning model sizes from 125M to a massive 180B.
To broaden the scope of the evaluation benchmarks, we focus on five different types of abilities in LLMs, including basic NLP abilities, emergent abilities, trustworthiness, dialogue, and long-context processing.
To investigate the effects of quantization on different tensor types, we evaluate the Weight-only, Weight-Activation, and KV Cache Quantization. 
%In addition, our evaluation incorporates a range of PTQ methods, including round-to-nearest (RTN), AWQ~\cite{AWQ}, and SmoothQuant~\cite{smoothquant}. 


% We open-source the evaluation and analysis tool to benefit future quantization applications and research\footnote{https://github.com/thu-nics/qllm-eval}. 
We summarize the key knowledge as shown in Table~\ref{tab:intro_knowledge}.
It's worth noting that \textit{we summarize many qualitative trends and failure cases that are common across different LLMs, which we conjecture to be general}.
However, \textit{the recommended bit-width may not generalize to other LLMs or tasks}.
% \vspace{-10pt}
% \begin{packed_itemize}
%     \item The larger the model, the higher the tolerance for Weight-only and KV Cache Quantization, while the tolerance for Activation Quantization is lower. 
%     % Additionally, we conducted a detailed analysis of this phenomenon by using statistical information.
%     % \item For the majority of models, the performance order of the quantized models is generally consistent with that of the original models.
%     \item Leveraging the Mixture-of-Experts (MoE) technique to increase the model size does not necessarily enhance the model’s tolerance to quantization.
%     \item For the majority of NLP tasks, quantizing most LLM families to W4, W4A8, KV4, and W8KV4 has negligible performance loss ($<2\%$). 
%     With a certain memory budget, employing larger models quantized to W3 yields superior performance.
%     \item Among four types of emergent abilities (i.e., in-context learning, instruction following, multi-step reasoning, and self-calibration), the self-calibration and multi-step reasoning abilities are more susceptible to quantization. For LLMs smaller than 13B, employing W8, W8A8, and KV8 quantization is recommended.
%     \item For ethics tasks, small models exhibit higher sensitivity to quantization. Weight-only Quantization amplifies the model's judgment of sensitive information, while KV Cache Quantization has the opposite effect.
%     \item The performance of LLMs on lengthy texts ($>$4k) is more sensitive to Weight-only and KV Cache Quantization than short texts ($<$4k), especially to the KV Cache Quantization. 
%     In most cases, W4, W4A8, and KV8 can sustain performance in long-context tasks.
%     \item The state-of-the-art (SOTA) quantization methods, such as SmoothQuant~\cite{smoothquant} and AWQ~\cite{AWQ}, can effectively enhance the performance when the performance loss brought by quantization is moderate. Nevertheless, when using extremely low bit-width, AWQ and SmoothQuant cannot restore the fully corrupted performances.
% \end{packed_itemize}

==> ICML24/Sections/limitation.tex <==
\section{Limitations}
\label{sec:limit}
In this paper, we focused solely on Post-training Quantization (PTQ) and did not consider Quantization-Aware Training (QAT).
Furthermore, we did not conduct detailed ablation studies on certain hyperparameters, such as investigating the effect of different group sizes in group-wise quantization. 
For certain types of LLMs (e.g., small LLMs with sizes between 1B to 3B), we did not evaluate all the newly available LLMs.
Some concrete recommendations on the bitwidth are specific to certain LLMs for certain tasks, and might not work well for new tasks and LLMs.

==> ICML24/Sections/pre.tex <==
\begin{table*}[h]
    \centering
    \caption{The benchmarks and model families for evaluation. ``Size'' represents the number of samples in the test set.}
    \vspace{-5pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c}
        \toprule
        Section & Tasks \& Ability & Benchmark & Size &  Model Family \\
        \midrule
         & \multirow{2}{*}{Language Modeling} & CHID~\cite{CHID} & 2002 &    \\
        \cmidrule{3-4}
         &  & Winogrande~\cite{winogrande} & 1267 &  \\
        \cmidrule{2-4}
         & \multirow{2}{*}{Understanding} & RACE~\cite{race} & 3489 &  OPT (125M-66B), LLaMA2 (7B-70B), \\
        \cmidrule{3-4}
        Sec.~\ref{sec:eval_basic} & &  LAMBADA~\cite{lambada} & 5153 & Falcon (7B-180B), Bloomz (560M-176B), \\
        % \cmidrule{3-4}
        % & & XSum~\cite{xsum} & 11300  & ChatGLM (6B) \\
        % \cmidrule{2-4}
        % &  & RTE~\cite{rte} & 3000 & \\
        \cmidrule{2-4}
        & \multirow{2}{*}{Reasoning} &  SIQA~\cite{siqa} & 1950 & Mistral(7B, 8$\times$7B)\\
        \cmidrule{3-4}
        &  &  PIQA~\cite{piqa} & 1876  & \\
        \midrule
        & \multirow{2}{*}{In-Context Learning} & MMLU~\cite{mmlu} & 14079 & \\
        \cmidrule{3-4}
        &  &  CEval~\cite{ceval} & 13948 & \\
        \cmidrule{2-4}
        Sec.~\ref{sec:eval_emergent} & \multirow{2}{*}{Multi-Step Reasoning} & GSM8K~\cite{gsm8k} & 1319 &  \\
        \cmidrule{3-4}
        &  &  StrategyQA~\cite{strategyqa} & 2290 & \\
        \cmidrule{2-4}
        & \multirow{2}{*}{Instruction-Following} & Hellaswag~\cite{hellaswag} &  10003 &  LLaMA2 (7B-70B), Falcon (7B-180B), \\
        \cmidrule{3-4}
        &  & ARC~\cite{arc-ec} & 7787 &  ChatGLM (6B), Mistral (7B, 8$\times$7B) \\
        \cmidrule{2-4}
        & Self-Calibration & MMLU~\cite{mmlu} & 14079 & Gemma (2B, 7B), Mamba (2.8B)\\
        \cmidrule{1-4}
        & Ethics & ETHICS~\cite{ethics} &  15160 & \\
        \cmidrule{2-4}
        Sec.~\ref{sec:eval_trust} & Hallucination & TruthfulQA~\cite{truthfulqa} &  817 & \\
        \cmidrule{2-4}
        & Robustness & AdvGLUE~\cite{advglue} &  738 & \\
        \cmidrule{1-4}\cdashline{5-5}
        Sec.~\ref{sec:eval_dia} & Dialogue & MT-bench~\cite{MT-bench} &  80 & (+ StableLM-3B)  \\
        \midrule
        \multirow{2}{*}{Sec.~\ref{sec:eval_long}} & \multirow{2}{*}{Long-Context} & Longeval~\cite{longchat} &  3000 & Vicuna (7B, 13B), LongChat (7B, 13B),  \\
        \cmidrule{3-4}
        &  & Multi-Doc QA~\cite{lost_in_the_middle} &  700 & ChatGLM (6B), Mistral (7B, 8$\times$7B)\\
        \bottomrule
    \end{tabular}}
    \label{tab:benchmark_ability_models}
\end{table*}

% \vspace{-10pt}
\section{Preliminaries}
\label{sec:pre}
\subsection{Quantization}
\label{sec:pre_quant}
% Quantization methods map a high-precision float-point value into discrete levels. 
In this paper, we focus on the most commonly used uniform quantization format~\cite{krishnamoorthi2018quantizing,nagel2021white},
whose quantization process can be expressed as:
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{Figures/pre/quant_grand.pdf}
  \end{center}
  % \vspace{-10pt}
  \caption{(a) Per-token quantization for Activation, (b) Group-wise quantization for Weight and KV Cache.}
  \label{fig:pre-quant_grand}
\end{figure}

\begin{equation}
\label{eq:integer_quant_main}
    \textbf{X}_{\mathrm{INT}} = \left[ \frac{\textbf{X}_{\mathrm{FP16}}-Z}{S} \right],
\end{equation}
\begin{equation}
\label{eq:integer_quant_scale}
    S = \frac{\mathrm{max}(\textbf{X}_{\mathrm{FP16}})-\mathrm{min}(\textbf{X}_{\mathrm{FP16}})}{2^{N-1}-1},
\end{equation}
% \begin{equation}
% \label{eq:integer_quant_zero}
%     Z = min(\textbf{X_{FP16}}),
% \end{equation}
where $X_{\mathrm{FP16}}$ denotes the 16-bit floating-point (FP16) value, $X_{\mathrm{INT}}$ denotes the low-precision integer value. 
$N$ is bit-width.
$S$ and $Z$ denote the scaling factor and zero-point. 
For symmetric quantization, the zero-point $Z$ is zero. 
For asymmetric quantization, we use $Z = \mathrm{min}(\textbf{X}_{\mathrm{FP16}})$. 


We study three different types of quantization:
(1) \textbf{Weight-only Quantization}: Only quantize the weight tensor $\textbf{W}$ of each linear layer. 
(2) \textbf{Weight-Activation Quantization}: Quantize both the input Activation $\textbf{X}$ and the Weight tensor $\textbf{W}$ of each linear layer.
(3) \textbf{KV Cache Quantization}: Quantize the key tensor $\textbf{K}$ and value tensor $\textbf{V}$ in each self-attention block.
For simplicity, we use W, A, and KV followed by a positive integer to indicate the quantization to a specific bit-width for Weight, Activation, and KV Cache, respectively. 
For example, W4A8 denotes quantizing Weights to 4-bit and Activations to 8-bit.

We quantize different tensors with different granularity levels. 
For Weight-only Quantization, we apply asymmetric group-wise quantization as shown in Figure~\ref{fig:pre-quant_grand} (b).
In this case, we split the Weight tensor into several groups with the same number of values.
In each group, we apply the asymmetric uniform quantization as shown in Equation~\ref{eq:integer_quant_main} and ~\ref{eq:integer_quant_scale}.
For Weight-Activation Quantization, we apply asymmetric group-wise quantization for the Weight tensors and use the symmetric per-token quantization for the Activation tensors as shown in Figure~\ref{fig:pre-quant_grand} (a). 
In this case, we share one scaling factor in each token.
For KV Cache Quantization, we apply the asymmetric group-wise quantization for both the Key and Value tensors.
See Appendix~\ref{app:exp_setup} for more details.



\subsection{Benchmarks and Models}
As illustrated in Table~\ref{tab:benchmark_ability_models}, we evaluate five distinct types of tasks in LLMs, including the basic NLP tasks in Sec.~\ref{sec:eval_basic}, the tasks for the emergent abilities in Sec.~\ref{sec:eval_emergent}, the trustworthiness tasks in Appendix~\ref{app:trust}, the dialogue tasks in Sec.~\ref{sec:eval_dia} and the long-context processing tasks in Sec.~\ref{sec:eval_long}. 
More details about datasets and evaluation workflows are in the Appendix.

For basic NLP tasks, we evaluate 5 LLM families, including the OPT~\cite{opt}, LLaMA2~\cite{llama2}, Falcon~\cite{falcon}, Bloomz~\cite{bloom}, ChatGLM~\cite{chatglm}, and Mistral~\cite{mistral} families. 
For the other four types of tasks, we mainly focus on evaluating the instruction-tuned Chatbot LLMs from the LLaMA2, Falcon, ChatGLM~\cite{chatglm}, and Mistral~\cite{mistral} families. 
In addition, we evaluate the emergent and dialogue ability of the latest StableLM-3B~\cite{StableLM}, Gemma~\cite{gemma}, and Mamba~\cite{mamba}.
To evaluate the long-context tasks, we choose the LLMs that support the long-context inference, including the Mistral and the ChatGLM families that support 32k context length, and the LongChat~\cite{longchat} and Vicuna~\cite{vicuna} families that support 16k context length.


\begin{figure*}[t]
% \vspace{-15pt}
% \vspace{-10pt}
    \centering
    \subfigure[W-only Quant.]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/basic/lambada_w_only.pdf}
    }%
    \centering
    \subfigure[WA Quant.]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/basic/lambada_w_a.pdf}
    }%
    \subfigure[KV Cache Quant.]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/basic/lambada_kv_cache.pdf}
    }%
    % \vspace{-10pt}
    \caption{The effect of quantization on different tensor types on LAMBADA (Natural Language Understanding task).}
    \label{fig:eval_basic_tensor_lambada}
\end{figure*}

\begin{figure*}[t]
    \centering
    \subfigure[LLaMA2 families on the RACE task]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/basic/llama2_race_storage_overhead.pdf}
    }%
    \centering
    \subfigure[Bloomz families on the RACE task]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/basic/bloomz_race_storage_overhead.pdf}
    }%
    \centering
    \subfigure[Bloomz families on the PIQA task]{
        \centering
        \includegraphics[width=0.33\linewidth]{Figures/basic/bloomz_piqa_storage_overhead.pdf}
    }%
    % \vspace{-10pt}
    \caption{Performances of the quantized LLMs with respect to their parameter scales. The parameter memory overheads are estimated by multiplying the parameter size by the quantization bit-width. The markers, $'\bullet', ~'\blacktriangle', ~'\blacksquare', ~'\blacklozenge', ~'+'$ denote the quantization bit-widths, W2, W3, W4, W8, FP16 respectively.}
    \label{fig:eval_basic_tasks}
\end{figure*}


\subsection{Statistical Analysis}
In this paper, we employ three tensor statistics to analyze the evaluation results. (1) The maximum absolute value (AbsMax) shows the dynamic range. (2) The standard deviation (Std) $\sigma$ reflects the extent to which data values deviate from the mean. A small standard deviation suggests that the tensor is more amenable to quantization. (3) The kurtosis $K=\frac{1}{n} \sum_{i=1}^{n} (\frac{x_i - \mu}{\sigma})^4$ summarizes the outlier condition of a certain tensor~\cite{kurtosis},
% \begin{equation}
%     K = \frac{1}{n} \sum_{i=1}^{n} (\frac{x_i - \mu}{\sigma})^4,
% \end{equation}
where $n$ is the number of data points in a tensor, and $\mu$ is the mean value of a tensor.
A high kurtosis indicates a distribution with heavy tails, indicating a higher likelihood of outliers.
%Kurtosis indicates the relative concentration of data in the tails of a distribution compared to the center. A large kurtosis indicates that the distribution has heavy tails, meaning it has a higher likelihood of outliers.
Conversely, a small kurtosis suggests light tails, indicating a distribution with fewer outliers.
% In addition, inspired by Xiao et al.~\cite{smoothquant}, where outliers in weights and activations are often concentrated in specific input channels, we also analyze the channel-wise min and max values of weights, activations, and KV Cache tensors. 


==> ICML24/Sections/related.tex <==
\section{Related Work}
\label{sec:rw}

==> Sections/conclusion.tex <==
% \vspace{-10pt}
\section{Conclusion and Potential Broader Impacts}
\label{sec:conclusion}
In this paper, we summarize the status quo of quantized LLMs.
Specifically, we summarize the phenomena of quantization on three tensor types, various LLM families, and different tasks.
Drawing from our evaluation results, we offer suggestions on how to choose and apply quantization techniques and point out the necessity of studying how to quantize MoE models and how to quantize models for long-context and math tasks. By presenting a thorough understanding of current trends, we expect our work to benefit future applications and research of LLM quantization. Our work also provides an early evaluation of the influences of efficiency techniques on trustworthiness, which is worth a more thorough investigation.

%Additionally, we point out directions to mitigate the bad effects of quantization on math, and long-context tasks and MoE models call for future work.

% Given our evaluations of various quantized LLMs on many tasks, we provide the following potential future directions to further explore the effects of quantization:
% (2) It is essential to explore how to reduce the performance loss of quantized models on more challenging tasks, such as mathematical reasoning tasks.
% (3) Further research is needed to delve into improving the performance of quantized models on long-text tasks, especially on KV Cache quantization.
% \todo{(1) Evaluations with more Quantization-Aware Training methods. Can specific abilities be preserved through QAT? }

% \todo{Code Generation task, QAT method Evaluation}

==> Sections/efficiency.tex <==
\section{Efficiency Analysis}
\label{sec:efficiency}

In this section, we discuss the efficiency bounds during the inference of LLMs. 
We need to quantize different tensor types to accelerate the operators with different bounds. 
Specifically, we use the Roofline model~\cite{roofline} to analyze the effect of quantizing different tensor types.

% \subsection{Analysis of the Latency Bound}
% \subsection{Analysis of the Memory Consumption}



==> Sections/related.tex <==
\section{Related Work}
\label{sec:rw}
